Quadratic Constraints for Local Stability Analysis of Quadratic Systems

This paper proposes new quadratic constraints (QCs) to bound a quadratic polynomial. Such QCs can be used in dissipation ineqaulities to analyze the stability and performance of nonlinear systems with quadratic vector fields. The proposed QCs utilize the sign-indefiniteness of certain classes of quadratic polynomials. These new QCs provide a tight bound on the quadratic terms along specific directions. This reduces the conservatism of the QC bounds as compared to the QCs in previous work. Two numerical examples of local stability analysis are provided to demonstrate the effectiveness of the proposed QCs.

==> Methods/CSQC.tex <==
\subsection{Properties of QC in Literature on Quadratic Monomials} \label{sec:CSQC}

Given a local region $\Ealpha$ and general quadratic nonlinearity, $\phi_i(x) = x^\top \hat{Q}_i x$, the following QC is proposed in~\cite{kalur2021LCSS}:
%
\begin{align} 
    \bmtx x \\ \phi_i \emtx^\top  
    \bmtx \alpha^2 (\hat{Q}_i E^{-1}\hat{Q}_i) & 0 \\ 0 & -1 \emtx
    \bmtx x \\ \phi_i \emtx \geq 0 & &  \forall x \in \Ealpha.
    \label{eq:CSQC}
\end{align}
%
By replacing $\bsmtx x \\ \phi_i \esmtx = \bsmtx I & 0 \\ 0 & b^\top \esmtx \bsmtx x \\ w \esmtx$, the QC~\eqref{eq:CSQC} recover the form in~\eqref{eq:QC}. Note that the QC~\eqref{eq:CSQC} corresponds to the inequality
\begin{align*}
    x^\top (\alpha^2 \hat{Q}_i E^{-1} \hat{Q}_i)x - \phi_i^2(x) \geq 0 & &  \forall x \in \Ealpha.
\end{align*}
To investigate the property of QC~\eqref{eq:CSQC}, we consider each case of possible quadratic monomials, $z_a(x) = x_i^2$ and $z_b(x) = x_ix_j$ where $i\neq j$. For simplicity, we consider the nonlinearity in the unit sphere ($E=I$ and $\alpha = 1$).

The QC~\eqref{eq:CSQC} of the case $z_a(x)=x_i^2$ corresponds to:
\begin{align}
    x_i^2 - z_a^2(x)\geq 0 & & \forall x^\top x \leq 1.     \label{eq:CSQC_phia}
\end{align} 
Fig.~\ref{fig:CSQC_PD} visualizes each term of the inequality in a three-dimensional space, where the horizontal axes are $x_i, x_j$ and the vertical axis is the function value. Note that $x_j$ is included while it is useful for discussion in the other case. One can observe that $x_i^2$ (blue surface) provides a reasonably well upper bound on $z_a^2(x)$ (green surface) over the local region. The QC~\eqref{eq:CSQC} can capture the local input-output behavior of the case $z_a(x)$ well over the region $\Ealpha$.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{Media/CSQC_za.png}
    \caption{Visualization of the QC~\eqref{eq:CSQC_phia}. The top subplot shows $z_a^2$ (green surface) where $z_a = x_i^2$ vs $(x_i,x_j)$. The plot also shows the blue surface ($x_i^2$) upper bounds the green on a unit sphere. The lower subplot shows the two function on the boundary of the unit sphere ($x^\top x=1$). The blue surface bounds the green reasonable well in the entire sphere.}
    \label{fig:CSQC_PD}
\end{figure}

On the other hand, QC~\eqref{eq:CSQC} fails to capture the case $z_b(x)$ along some directions. the QC~\eqref{eq:CSQC} of the case $z_b(x)$ corresponds to the inequality:
\begin{align}
    0.25(x_i^2+x_j^2) - z_b^2(x) \geq 0 & & \forall x^\top x\leq 1.  \label{eq:CSQC_phib}
\end{align}
 Fig.~\ref{fig:CSQC_zb} visualizes each term of the inequality. The landscape of $z_b^2(x)$ has peaks along the directions $x_i=\pm x_j$ and valleys along $z_b(x) = 0$ ($x_i=0$ and $x_j=0$). The function $0.25(x_i^2 + x_j^2)$ (blue surface) provides a tight upper bound of $z_b^2(x)$ (green surface) along peaks. However, the blue surface provides a loose bound along the valleys of green surface.

We note that these valleys are an inherent feature of a sign-indefinite monomial. Hence, the loose bound of CSQC does not depend on the shape and the size of the ellipsoidal region $\Ealpha$. Furthermore, this looseness will potentially lead to conservative analysis results as mentioned before. 

\begin{figure}[h]
    \centering
    \includegraphics[width=0.99\linewidth]{Media/CSQC_zb.png}
    \caption{Visualization of the QC~\eqref{eq:CSQC_phib}. The top subplot shows $z_b^2$ (green surface) where $z_k = x_ix_j$ vs $(x_i,x_j)$. The plot also shows the blue surface ($0.25(x_i^2+x_j^2)$) upper bounds the green on a unit sphere. The lower subplot shows the two function on the boundary of the unit sphere $(x^\top x=1)$. The blue surface tightly bounds the green only at the peaks but provides a loose bound at the valleys.}
    \label{fig:CSQC_zb}
\end{figure}



==> Methods/ProofingLemmas.tex <==
\subsection{Proofing Lemmas}

\begin{lemma}
    Let $E=E^\top\succ 0, \alpha>0$ be given and define a local ellipsoid $\mathcal{E}_\alpha = \{x\in\mathbb{R}^n : x^\top Ex \leq \alpha^2\}$. The following is true for any vector $c\in\mathbb{R}^n$:
    %
    \begin{align}
        \alpha^2(c^\top E^{-1} c) = &\max  (c^\top x)^2 \\
        &\mbox{s.t. } x\in\mathcal{E}_\alpha.
    \end{align}
    %
    If $c$ is a standard basis vector $e_i$, then $c^\top E^{-1}c = (E^{-1})_{ii}$ is the $(i,i)$ entry of $E^{-1}$.
\end{lemma}
%
\begin{proof}
    Define $w := E^{\frac{1}{2}}x$. The optimization problem can be reformed as maximizing $(c^\top E^{-\frac{1}{2}}w)^2$ over w subject to $w^\top w \leq \alpha^2$. By Cauchy-Schwartz ineqaulity:
    \begin{align*}
        (c^\top E^{-\frac{1}{2}}w)^2 &\leq \norm{E^{-\frac{1}{2}}c}^2_2 \cdot \norm{w}^2_2 \\
        &\leq \alpha^2 (c^\top E^{-1}c)
    \end{align*} 
    %
    Furthermore, $c^\top E c = e_i^\top E^{-1} e_i = (E^{-1})_{ii}$ is the $(i,i)$ entry of $E^{-1}$ when $c$ is a standard basis vector $e_i \in \mathbb{R}^n$.
\end{proof}



% right before rank-3 
\begin{lemma}
    Let $E=E^\top\succ 0, \alpha>0$ be given and define a local ellipsoid $\mathcal{E}_\alpha = \{x\in\mathbb{R}^n : x^\top Ex \leq \alpha^2\}$. The following is true for any symmetric matrix $Q=Q^\top \in\mathbb{R}^{n\times n}$ with at least one positive eigenvalue:
    %
    \begin{align}
        \alpha^2\lambda_{max}(E^{-\frac{1}{2}}QE^{-\frac{1}{2}}) = &\max x^\top Q x \\
        &\mbox{s.t. } x\in\mathcal{E}_\alpha
    \end{align}
\end{lemma}
%
\begin{proof}
    Let $T\Lambda T^\top = E^{-\frac{1}{2}}QE^{-\frac{1}{2}}$ be the eigendecomposition and define $w := \frac{1}{\alpha}TE^{\frac{1}{2}}x$. The optimization problem can be reformed as maximizing $\alpha^2w^\top\Lambda w$ over $w$ subject to $w^\top w \leq 1$. Note that $\Lambda$ has at least one positive eigenvalue as $Q$ has since $E^{\frac{1}{2}}$ is positive definite. The lemma follows as $w^\top\Lambda w$ is less than the largest eigenvalue of $\Lambda$ for all $w^\top w \leq 1$.
\end{proof}


